Infinity-Norm Sphere-Decoding

The most promising approaches for efficient detection in multiple-input multiple-output (MIMO) wireless systems are based on sphere-decoding (SD). The conventional (and optimum) norm that is used to conduct the tree traversal step in SD is the l-2 norm. It was, however, recently observed that using the l-infinity norm instead reduces the hardware complexity of SD considerably at only a marginal performance loss. These savings result from a reduction in the length of the critical path in the circuit and the silicon area required for metric computation, but are also, as observed previously through simulation results, a consequence of a reduction in the computational (i.e., algorithmic) complexity. The aim of this paper is an analytical performance and computational complexity analysis of l-infinity norm SD. For i.i.d. Rayleigh fading MIMO channels, we show that l-infinity norm SD achieves full diversity order with an asymptotic SNR gap, compared to l-2 norm SD, that increases at most linearly in the number of receive antennas. Moreover, we provide a closed-form expression for the computational complexity of l-infinity norm SD based on which we establish that its complexity scales exponentially in the system size. Finally, we characterize the tree pruning behavior of l-infinity norm SD and show that it behaves fundamentally different from that of l-2 norm SD.

==> LinfSD_sub.bbl.tex <==
\begin{thebibliography}{10}

\bibitem{rohit03}
A.~Paulraj, R.~Nabar, and D.~Gore, {\em Introduction to Space-Time Wireless
  Communications}.
\newblock Cambridge (UK): Cambridge Univ. Press, 2003.

\bibitem{burg_phd}
A.~Burg, {\em {VLSI} {C}ircuits for {MIMO} {C}ommunication {S}ystems}.
\newblock Konstanz: Hartung-Gorre Verlag, 2006.

\bibitem{fincke_phost85}
U.~Fincke and M.~Pohst, ``Improved methods for calculating vectors of short
  length in a lattice, including a complexity analysis,'' {\em Math. Comp.},
  vol.~44, pp.~463--471, Apr. 1985.

\bibitem{viterbo93}
E.~Viterbo and E.~Biglieri, ``A universal decoding algorithm for lattice
  codes,'' in {\em GRETSI 14-\`eme Colloq.}, (Juan-les-Pins, France),
  pp.~611--614, Sept. 1993.

\bibitem{agrell_it02}
E.~Agrell, T.~Eriksson, A.~Vardy, and K.~Zeger, ``Closest point search in
  lattices,'' {\em IEEE Trans. Inf. Theory}, vol.~48, no.~8, pp.~2201--2214, Aug.
  2002.

\bibitem{damen03}
M.~O. Damen, H.~{El Gamal}, and G.~Caire, ``On maximum-likelihood detection and
  the search for the closest lattice point,'' {\em IEEE Trans. Inf. Theory},
  vol.~49, no.~10, pp.~2389--2402, Oct. 2003.

\bibitem{burg05_vlsi}
A.~Burg, M.~Borgmann, M.~Wenk, M.~Zellweger, W.~Fichtner, and {H.\ B\"olcskei},
  ``{VLSI} implementation of {MIMO} detection using the sphere decoding
  algorithm,'' {\em IEEE J. of Solid-State Circuits}, vol.~40, no.~7, pp.~1566--1577,
  July 2005.

\bibitem{studer08}
C.~Studer, A.~Burg, and H.~B\"olcskei, ``Soft-output sphere decoding:
  {A}lgorithms and {VLSI} implementation,'' {\em IEEE J. on Select. Areas in
  Comm.}, vol.~26, no.~2, pp.~290--300, Feb.\ 2008.

\bibitem{hass_sp03_part_i}
B.~Hassibi and H.~Vikalo, ``On the sphere decoding algorithm {I}. {E}xpected
  complexity,'' {\em IEEE Trans. Signal Processing}, vol.~53, no.~8, pp.~2806--2818,
  Aug. 2005.

\bibitem{kaeslin08}
H.\ Kaeslin, {\em Digital Integrated Circuit Design: From VLSI Architectures to CMOS Fabrication}. \newblock Cambridge (UK): Cambridge Univ. Press, 2008.

\bibitem{hass_sp03_part_ii}
H.~Vikalo and B.~Hassibi, ``On the sphere decoding algorithm {II}.
  {G}eneralizations, second-order statistics, and applications to
  communications,'' {\em IEEE Trans. Signal Processing}, vol.~53, no.~8,  
  pp.~2819--2834, Aug. 2005.

\bibitem{murugan06}
A.~D. Murugan, H.~{El Gamal}, M.~O. Damen, and G.~Caire, ``A unified framework
  for tree search decoding: {R}ediscovering the sequential decoder,'' {\em IEEE
  Trans. Inform. Theory}, vol.~52, no.~3, pp.~933--953, Mar. 2006.

\bibitem{Gowaikar_07}
R.~Gowaikar and B.~Hassibi, ``Statistical pruning for near-maximum likelihood
  decoding,'' {\em IEEE Trans. Signal Processing}, vol.~55, no.~6, pp.~2661--2675,
  June 2007.

\bibitem{jalden_tsp05}
J.~Jald\'en and B.~Ottersten, ``On the complexity of sphere decoding in digital
  communications,'' {\em IEEE Trans. Signal Processing}, vol.~53, no.~4, 
  pp.~1474--1484, Apr. 2005.

\bibitem{papoulis91}
A.~Papoulis, {\em Probability, Random Variables, and Stochastic Processes}.
\newblock New York: McGraw-Hill, 3rd~ed., 1991.

\bibitem{Knuth_76}
D.~E. Knuth, ``Big omicron and big omega and big theta,'' {\em Association for
  Computing Machinery SIGACT News}, vol.~8, no.~2, pp.~18--24, 1976.

\bibitem{hochbrink03}
B.~M. Hochwald and S.~{ten Brink}, ``Achieving near-capacity on a
  multiple-antenna channel,'' {\em IEEE Trans. Inf. Theory}, vol.~51, no.~3, 
  pp.~389--399, Mar. 2003.

\bibitem{banih_98}
A.~H. Banihashemi and A.~K. Khandani, ``On the complexity of decoding lattices
  using the {K}orkin-{Z}olotarev reduced basis,'' {\em IEEE Trans. Inf.
  Theory}, vol.~44, no.~1, pp.~162--171, Jan. 1998.

\bibitem{babai86}
L.~Babai, ``On {L}ov\'asz' lattice reduction and the nearest lattice point
  problem,'' {\em Combinatorica}, vol.~6, pp.~1--13, 1986.

\bibitem{tarokh_it98}
V.~Tarokh, N.~Seshadri, and A.~R. Calderbank, ``Space-time codes for high data
  rate wireless communications: {P}erformance criterion and code
  construction,'' {\em IEEE Trans. Inf. Theory}, vol.~44, no.~2, pp.~744--765, Mar.
  1998.

\bibitem{zheng02}
L.~Zheng and D.~Tse, ``Diversity and multiplexing: A fundamental tradeoff in
  multiple antenna channels,'' {\em IEEE Trans. Inf. Theory}, vol.~49, no.~5, 
  pp.~1073--1096, May 2003.

\bibitem{loyka04}
S.~Loyka and F.~Gagnon, ``Performance analysis of the {V-BLAST} algorithm: {A}n
  analytical approach,'' {\em IEEE Trans. Wireless Comm.}, vol.~3, no.~4, 
  pp.~1326--1337, Jul.\ 2004.

\bibitem{lu_wang_kumar_chugg03}
H.~Lu, Y.~Wang, P.~V. Kumar, and K.~M. Chugg, ``Remarks on space-time codes
  including a new lower bound and an improved code,'' {\em IEEE Trans. Inf.
  Theory}, vol.~49, no.~10, pp.~2752--2757, Oct. 2003.

\bibitem{jalden_icassp08i}
J.~Jald\'en and G.~Matz, ``{MIMO} receiver diversity in general fading,'' in
  {\em Proc. {IEEE} ICASSP 2008}, (Las Vegas, NV), pp.~2837--2840, Mar./Apr.
  2008.

\bibitem{tulino04}
A.~M. Tulino and S.~Verd\'u, {\em Random Matrix Theory and Wireless
  Communications}.
\newblock Hanover, MA: Now Publishers Inc.\, 2004.

\bibitem{behboodian72}
J.~Behboodian, ``On the distribution of a symmetric statistic from a mixed
  population,'' {\em Technometrics}, vol.~14, no.~4, pp.~919--923, Nov. 1972.

\bibitem{damen00}
M.~O. Damen, A.~Chkeif, and J.~C. Belfiore, ``Lattice code decoder for space-time
  codes,'' {\em IEEE Comm. Letters}, vol.~4, no.~5, pp.~161--163, May 2000.

\bibitem{jalden_ISIT05}
J.~Jald\'en and B.~Ottersten, ``On the limits of sphere decoding,'' 
in {\em Proc. {IEEE} {ISIT} 2005}, (Adelaide, Australia), pp.~1691--1695, Sept. 2005.

\bibitem{david03}
H.~A. David and H.~N. Nagaraja, {\em Order Statistics}.
\newblock Hoboken, New Jersey: Wiley, 3rd~ed., 2003.

\bibitem{Finch_03}
S.~R. Finch, {\em Mathematical Constants}.
\newblock Cambridge (UK): Cambridge Univ. Press, 2003.

\bibitem{ball_97}
K.~Ball, ``An elementary introduction to modern convex geometry,'' {\em in MSRI
  book series, Flavors of Geometry, {\em Cambridge (UK): Cambridge Univ.
  Press}}, vol.~31, pp.~1--58, 1997.

\bibitem{muir05}
R.~J. Muirhead, {\em Aspects of Multivariate Statistical Theory}.
\newblock Hoboken, New Jersey: Wiley, 2005.

\bibitem{Abr65}
M.~Abramowitz and I.~Stegun, {\em Handbook of Mathematical Functions}.
\newblock New York: Dover, 1965.

\bibitem{gautschi98}
W.~Gautschi, ``The incomplete gamma functions since {T}ricomi,'' {\em In
  Tricomi's Ideas and Contemporary Applied Mathematics}, pp.~203--237, 1998.

\bibitem{merkle_93}
M.~Merkle, ``Some inequalities for the chi square distribution function and the
  exponential function,'' {\em Arch. Math.}, vol.~60, no.~5, pp.~451--458,
  1993.

\bibitem{boyd_conv_opt01}
S.~Boyd and L.~Vandenberghe, {\em Convex Optimization}.
\newblock Cambridge (UK): Cambridge Univ. Press, Dec. 2004.

\bibitem{Bagnoli05}
M.~Bagnoli and T.~Bergstrom, ``Log-concave probability and its applications,''
  {\em Economic Theory}, vol.~26, no.~2, pp.~445--469, Aug. 2005.

\end{thebibliography}

